Bayesian latent hierarchical model for transcriptomic meta-analysis to detect biomarkers with clustered meta-patterns of differential expression signals

Due to the rapid development of high-throughput experimental techniques and fast-dropping prices, many transcriptomic datasets have been generated and accumulated in the public domain. Meta-analysis combining multiple transcriptomic studies can increase the statistical power to detect disease-related biomarkers. In this paper, we introduce a Bayesian latent hierarchical model to perform transcriptomic meta-analysis. This method is capable of detecting genes that are differentially expressed (DE) in only a subset of the combined studies, and the latent variables help quantify homogeneous and heterogeneous differential expression signals across studies. A tight clustering algorithm is applied to detected biomarkers to capture differential meta-patterns that are informative to guide further biological investigation. Simulations and three examples, including a microarray dataset from metabolism-related knockout mice, an RNA-seq dataset from HIV transgenic rats, and cross-platform datasets from human breast cancer, are used to demonstrate the performance of the proposed method.

==> pictureV3/simulation/basic/simulationSummary/S10/ndet__S10_.tex <==
 & 1 &   237 (   14) &   623 (   27) &  2937 (   20) &  2851 (   20) &  2883 (   22) &  1331 (   29) &  1845 (   32)\\
 & 2 &   102 (   11) &   369 (   22) &  2179 (   33) &  2021 (   32) &  2014 (   34) &   916 (   23) &  1287 (   33)\\
 & 3 &    22 (    6) &   166 (   16) &  1529 (   34) &  1240 (   31) &  1177 (   35) &   636 (   17) &   740 (   28)\\


==> pictureV3/simulation/basic/simulationSummary/S3/ndet__S3_.tex <==
 & 1 &   828 (   23) &  1075 (   30) &  2725 (   25) &  2671 (   25) &  2683 (   24) &  1741 (   31) &  1905 (   33)\\
 & 2 &   411 (   19) &   607 (   26) &  1662 (   37) &  1518 (   34) &  1499 (   34) &  1021 (   26) &  1089 (   32)\\
 & 3 &   132 (   14) &   248 (   20) &   843 (   34) &   662 (   32) &   609 (   30) &   488 (   21) &   451 (   25)\\


==> pictureV3/simulation/basic/simulationSummary/S5/ndet__S5_.tex <==
 & 1 &   480 (   21) &   801 (   31) &  2811 (   24) &  2748 (   22) &  2770 (   24) &  1581 (   30) &  1863 (   35)\\
 & 2 &   223 (   15) &   464 (   24) &  1864 (   35) &  1718 (   33) &  1696 (   34) &  1004 (   27) &  1167 (   33)\\
 & 3 &    63 (    9) &   202 (   18) &  1109 (   39) &   881 (   34) &   814 (   32) &   579 (   23) &   564 (   30)\\


==> pictureV3/simulation/cluster12/mainClustering/alphaLevel0.05/tightcos/aks6/tightZ_table.tex <==
1 & 18 & 22 & 0 & 0 & 0 & \textbf{82} & 6\\
2 & 21 & 21 & \textbf{65} & 0 & 0 & 0 & 2\\
3 & 13 & 15 & 0 & \textbf{69} & 0 & 0 & 3\\
4 & 11 & 14 & 0 & 1 & \textbf{67} & 0 & 3\\
5 & \textbf{17} & 15 & 0 & 1 & 0 & 0 & 3\\
6 & \textbf{18} & 15 & 0 & 0 & 0 & 0 & 2\\
0 & \textbf{86} & 72 & 1 & 1 & 2 & 2 & 12\\


==> pictureV3/simulation/correlatedNull/simulationSummary/S3/aucClustSize.tex <==
 & 200 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 300 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 400 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 500 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\


==> pictureV3/simulation/correlatedNull/simulationSummary/S3/fdrClustSize.tex <==
 & 200 & 0.058 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\
 & 300 & 0.057 (0.008) & 0.041 (0.004) & 0.034 (0.004)\\
 & 400 & 0.057 (0.009) & 0.041 (0.005) & 0.034 (0.004)\\
 & 500 & 0.058 (0.009) & 0.041 (0.005) & 0.034 (0.004)\\


==> pictureV3/simulation/correlatedNull/simulationSummary/S3/fnrClustSize.tex <==
 & 200 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 300 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 400 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 500 & 0.024 (0.002) & 0.053 (0.002) & 0.039 (0.002)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenBoth/auc_unevenBoth.tex <==
0.988 & 0.927 & 0.987 & 0.986 & 0.987 & 0.991 & 0.986\\
&& (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.001) & (0.002)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenBoth/fdr_unevenBoth.tex <==
0.052 & 0.207 & 0.044 & 0.035 & 0.036 & 0.035 & 0.090\\
&& (0.007) & (0.012) & (0.003) & (0.004) & (0.004) & (0.004) & (0.007)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenBoth/fnr_unevenBoth.tex <==
0.015 & 0.009 & 0.028 & 0.031 & 0.029 & 0.021 & 0.017\\
&& (0.001) & (0.001) & (0.002) & (0.002) & (0.002) & (0.002) & (0.001)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenSampleSize/AUC_unevenSampleSize.tex <==
0.985 & 0.927 & 0.985 & 0.984 & 0.985 & 0.989 & 0.984\\
&& (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.001) & (0.002)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenSampleSize/fdr_unevenSampleSize.tex <==
0.053 & 0.205 & 0.043 & 0.035 & 0.035 & 0.034 & 0.087\\
&& (0.006) & (0.013) & (0.004) & (0.004) & (0.004) & (0.004) & (0.007)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenSampleSize/fnr_unevenSampleSize.tex <==
0.016 & 0.010 & 0.032 & 0.035 & 0.033 & 0.024 & 0.019\\
&& (0.001) & (0.001) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenStudySampleSize234/AUC_unevenStudySampleSize234.tex <==
0.986 & 0.928 & 0.984 & 0.983 & 0.984 & 0.988 & 0.982\\
&& (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.001) & (0.002)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenStudySampleSize234/fdr_unevenStudySampleSize234.tex <==
0.054 & 0.206 & 0.044 & 0.035 & 0.035 & 0.034 & 0.088\\
&& (0.008) & (0.013) & (0.004) & (0.004) & (0.004) & (0.004) & (0.007)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenStudySampleSize234/fnr_unevenStudySampleSize234.tex <==
0.017 & 0.012 & 0.034 & 0.037 & 0.035 & 0.026 & 0.021\\
&& (0.001) & (0.001) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenStudySampleSize2510/AUC_unevenStudySampleSize2510.tex <==
0.993 & 0.926 & 0.991 & 0.990 & 0.990 & 0.995 & 0.988\\
&& (0.001) & (0.002) & (0.001) & (0.001) & (0.001) & (0.001) & (0.002)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenStudySampleSize2510/fdr_unevenStudySampleSize2510.tex <==
0.051 & 0.209 & 0.049 & 0.035 & 0.035 & 0.037 & 0.089\\
&& (0.006) & (0.012) & (0.003) & (0.004) & (0.004) & (0.003) & (0.007)\\


==> pictureV3/simulation/sampleSizes/Summary/unevenStudySampleSize2510/fnr_unevenStudySampleSize2510.tex <==
0.012 & 0.009 & 0.019 & 0.022 & 0.021 & 0.015 & 0.014\\
&& (0.001) & (0.001) & (0.002) & (0.002) & (0.002) & (0.001) & (0.001)\\


==> pictureV3/simulation/sensitivityAnalysis/summary/AUCAlpha.tex <==
 & 0.1 & 0.975 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 0.5 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 1 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 5 & 0.977 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 10 & 0.977 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\


==> pictureV3/simulation/sensitivityAnalysis/summary/AUCsigma0.tex <==
 & 5 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 10 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 15 & 0.976 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 20 & 0.975 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 25 & 0.975 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\
 & 30 & 0.975 (0.003) & 0.973 (0.002) & 0.980 (0.002)\\


==> pictureV3/simulation/sensitivityAnalysis/summary/fdrAlpha.tex <==
 & 0.1 & 0.057 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\
 & 0.5 & 0.058 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\
 & 1 & 0.058 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\
 & 5 & 0.059 (0.008) & 0.042 (0.004) & 0.035 (0.004)\\
 & 10 & 0.059 (0.008) & 0.042 (0.004) & 0.035 (0.004)\\


==> pictureV3/simulation/sensitivityAnalysis/summary/fdrsigma0.tex <==
 & 5 & 0.059 (0.008) & 0.042 (0.004) & 0.035 (0.004)\\
 & 10 & 0.058 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\
 & 15 & 0.058 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\
 & 20 & 0.058 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\
 & 25 & 0.058 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\
 & 30 & 0.058 (0.008) & 0.042 (0.004) & 0.034 (0.004)\\


==> pictureV3/simulation/sensitivityAnalysis/summary/fnrAlpha.tex <==
 & 0.1 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 0.5 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 1 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 5 & 0.024 (0.002) & 0.053 (0.003) & 0.039 (0.002)\\
 & 10 & 0.024 (0.002) & 0.053 (0.003) & 0.039 (0.002)\\


==> pictureV3/simulation/sensitivityAnalysis/summary/fnrsigma0.tex <==
 & 5 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 10 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 15 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 20 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 25 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\
 & 30 & 0.024 (0.002) & 0.054 (0.003) & 0.039 (0.002)\\

